Patch-Fool: Are Vision Transformers Always Robust Against Adversarial Perturbations?

Vision transformers (ViTs) have recently set off a new wave in neural architecture design thanks to their record-breaking performance in various vision tasks. In parallel, to fulfill the goal of deploying ViTs into real-world vision applications, their robustness against potential malicious attacks has gained increasing attention. In particular, recent works show that ViTs are more robust against adversarial attacks as compared with convolutional neural networks (CNNs), and conjecture that this is because ViTs focus more on capturing global interactions among different input/feature patches, leading to their improved robustness to local perturbations imposed by adversarial attacks. In this work, we ask an intriguing question: "Under what kinds of perturbations do ViTs become more vulnerable learners compared to CNNs?" Driven by this question, we first conduct a comprehensive experiment regarding the robustness of both ViTs and CNNs under various existing adversarial attacks to understand the underlying reason favoring their robustness. Based on the drawn insights, we then propose a dedicated attack framework, dubbed Patch-Fool, that fools the self-attention mechanism by attacking its basic component (i.e., a single patch) with a series of attention-aware optimization techniques. Interestingly, our Patch-Fool framework shows for the first time that ViTs are not necessarily more robust than CNNs against adversarial perturbations. In particular, we find that ViTs are more vulnerable learners compared with CNNs against our Patch-Fool attack which is consistent across extensive experiments, and the observations from Sparse/Mild Patch-Fool, two variants of Patch-Fool, indicate an intriguing insight that the perturbation density and strength on each patch seem to be the key factors that influence the robustness ranking between ViTs and CNNs.

==> Section/3-Sanity-Check.tex <==
% \section{Benchmark the robustness of ViTs and CNNs under existing attacks}
\vspace{-0.5em}
\section{Evaluating robustness of ViTs and CNNs under existing attacks}
\vspace{-0.5em}
\label{sec:sanity-check}
% In this section, we conduct a sanity check on the benchmark of the adversarial robustness between several representative ViT variants and SOTA CNN models with comparable complexities against existing white-box attacks.

% Although the comparisons between the robustness of ViTs and CNNs have been explored in pioneering works~\citep{bhojanapalli2021understanding, aldahdooh2021reveal, shao2021adversarial}, their evaluation suffers from one of the several limitations: (1) only adopt weak attack methods, (2) only adopt early ViT designs without considering recent advances in ViTs' architectures, and (3) do not adopt official and latest pretrained models and suffer from inferior clean accuracy. To this end, we extensively evaluate the robustness against common white-box attacks of several representative ViT variants, which cover the popular trends in designing ViT architectures, including (1) using local self-attention (Swin~\citep{liu2021swin}), which adopts the attention mechanism within a local region instead of global ones in vanilla ViTs to capture low-level features and reduce the computationsl cost, and (2) introducing the inductive bias of CNNs to build hybrid models (LeViT~\citep{graham2021levit}).
Although various comparisons on robustness of ViTs and CNNs have been explored in pioneering works~\citep{bhojanapalli2021understanding, aldahdooh2021reveal, shao2021adversarial}, their evaluation suffers from one of the following limitations: (1) only adopt weak attack methods, (2) only adopt early ViT designs without considering recently advanced ViT architectures, and (3) do not adopt the official and latest pretrained models and suffer from inferior clean accuracies. To this end, we extensively evaluate the robustness against common white-box attacks of several representative ViT variants, which cover the popular trends in designing ViT architectures, including (1) using local self-attention (Swin~\citep{liu2021swin}), which adopts the attention mechanism within a local region instead of the global ones in vanilla ViTs to capture low-level features and reduce the computational cost, and (2) introducing the inductive bias of CNNs to build hybrid models (LeViT~\citep{graham2021levit}).


\begin{table}[th]
\centering
% \caption{Benchmark the robustness of three ViT families and two CNN families against PGD attacks~\citep{madry2017towards}, Auto-Attack~\citep{croce2020reliable}, and CW attacks~\citep{carlini2017towards}. The perturbation strengths of the L-inf attacks are annotated.}
\vspace{-0.5em}
\caption{Benchmark the robustness of three ViT families and two CNN families against PGD attacks~\citep{madry2017towards}, Auto-Attack~\citep{croce2020reliable}, and CW attacks~\citep{carlini2017towards}, where the perturbation strengths of the L-inf attacks are annotated.}
\vspace{-0.5em}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{ccc||ccc||cc||ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}FLOPs/\\ Params\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Clean \\ Acc (\%)\end{tabular}}} & \multicolumn{3}{c||}{\textbf{PGD-20 (\%)}} & \multicolumn{2}{c||}{\textbf{Auto-Attack (\%)}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}CW-$L_{2}$ \\ (\%)\end{tabular}}}} & \multicolumn{2}{c}{\textbf{CW-$L_{Inf}$ (\%)}} \\
 &  &  & \textbf{0.001} & \textbf{0.003} & \textbf{0.005} & \textbf{0.001} & \textbf{0.003} & \multicolumn{1}{c}{} & \textbf{0.003} & \textbf{0.005} \\ \midrule
ResNet-18 & 1.80G/23M & 71.78 & 22.60 & 0.34 & 0.00 & 22.29 & 0.06 & 9.95 & 9.10 & 5.31 \\
ResNet-50 & 4.11G/98M & 76.15 & 35.00 & 1.42 & 0.18 & 25.42 & 1.23 & 10.80 & 13.39 & 7.95 \\
ResNet-101 & 7.83G/170M & 78.25 & 37.20 & 2.10 & 0.42 & 27.92 & 1.88 & 11.19 & 15.36 & 11.11 \\
ResNet-152 & 11.56G/230M & 78.31 & 42.09 & 2.56 & 0.24 & 39.58 & 2.34 & 15.20 & 17.24 & 14.58 \\
\midrule
VGG-16 & 15.3G/134M & 71.30 & 23.24 & 0.28 & 0.02 & 15.42 & 0.04 & 8.15 & 7.84 & 4.84 \\ \midrule
\midrule
DeiT-Ti & 1.26G/5M & 72.02 & 41.51 & 6.73 & 1.52 & 38.29 & 5.75 & 30.08 & 28.74 & 21.05 \\
DeiT-S & 4.61G/22M & 79.53 & 53.70 & 11.40 & 2.91 & 51.88 & 7.70 & 43.78 & 44.22 & 34.65 \\
DeiT-B & 17.58G/86M & 81.90 & 52.20 & 10.10 & 2.28 & 51.08 & 8.62 & 43.77 & 47.40 & 36.35 \\
\midrule
Swin-T & 4.51G/29M & 80.96 & 38.80 & 2.72 & 1.08 & 35.81 & 2.04 & 28.84 & 35.10 & 20.63 \\
Swin-S & 8.77G/50M & 82.37 & 47.20 & 6.79 & 0.42 & 43.25 & 4.58 & 30.32 & 41.22 & 28.91 \\
Swin-B & 15.47G/88M & 84.48 & 47.16 & 7.30 & 1.14 & 44.58 & 6.52 & 34.34 & 43.57 & 34.00 \\
\midrule
LeViT-256 & 1.13G/19M & 81.60 & 36.42 & 3.00 & 0.64 & 31.25 & 2.29 & 43.94 & 46.57 & 25.58 \\
LeViT-384 & 2.35G/39M & 82.60 & 42.19 & 3.08 & 0.24 & 35.83 & 2.50 & 47.15 & 50.22 & 39.56 \\ 
\bottomrule
\end{tabular}
}
\vspace{-1em}
\label{tab:sanity_check}%
\end{table}%



% \subsection{Whether ViTs are more robust than CNNs?}
% \label{sec:benchmark}


% \subsection{Setup} 
\vspace{-0.5em}
\subsection{Evaluation Setup} 
\vspace{-0.5em}
\label{sec:sanity_check_setup}

% \textbf{Models and datasets.}
% We evaluate the robustness of three ViT families (DeiT~\citep{touvron2021training}, Swin~\citep{liu2021swin}, LeViT~\citep{graham2021levit}) and two CNN families (ResNet~\citep{he2016deep}, and VGG~\citep{simonyan2014very}) on ImageNet with official implementation and pretrained models. Note that we adopt DeiT models without distillation for a fair comparison, which only improves the training schedule over vanilla ViTs.

% \textbf{Attack settings.}
% We adopt four adversarial attacks (PGD~\citep{madry2017towards}, AutoAttack~\citep{croce2020reliable}, CW-$L_{Inf}$~\citep{carlini2017towards}, CW-$L_{2}$) with different perturbation strengths. In particular, for the CW-$L_{Inf}$ and CW-$L_{2}$ attacks we adopt the implementation in AdverTorch~\citep{ding2019advertorch} and the same settings in~\citep{chen2021robust, rony2019decoupling}. For AutoAttack, we adopt the official implementation and default settings in~\citep{croce2020reliable}.

\textbf{Models and datasets.}
We evaluate the robustness of three ViT families (i.e., DeiT~\citep{touvron2021training}, Swin~\citep{liu2021swin}, and LeViT~\citep{graham2021levit}) and two CNN families (ResNet~\citep{he2016deep} and VGG~\citep{simonyan2014very}) on ImageNet using their official implementation and pretrained models. Note that we adopt DeiT models without distillation, which only improves the training schedule over vanilla ViTs, for a fair comparison.

\textbf{Attack settings.}
We adopt four adversarial attacks (i.e., PGD~\citep{madry2017towards}, AutoAttack~\citep{croce2020reliable}, CW-$L_{Inf}$~\citep{carlini2017towards}, and CW-$L_{2}$) with different perturbation strengths. In particular, for the CW-$L_{Inf}$ and CW-$L_{2}$ attacks, we adopt the implementation in AdverTorch~\citep{ding2019advertorch} and the same settings as~\citep{chen2021robust, rony2019decoupling}; For AutoAttack, we adopt the official implementation and default settings in~\citep{croce2020reliable}.

\vspace{-0.5em}
\subsection{Observations and analysis}
\vspace{-0.5em}
% \textbf{Observations.} As shown in Tab.~\ref{tab:sanity_check}, we make the following observations: (1)ViTs are consistently more robust than CNNs with comparable model complexities under all attack methods, which is consistent with the previous observations~\citep{bhojanapalli2021understanding, aldahdooh2021reveal, shao2021adversarial}. In particular,DeiT-S/DeiT-B achieves a 18.70\%/10.11\% higher robust accuracy over ResNet-50/ResNet-152 under PGD-20 attacks with a perturbation strength of 0.001; (2) compared with vanilla ViTs, variants equipped with local self-attention or convolutional modules, which improves the capability to capture local features thus boosts the clean accuracy, are more vulnerable to adversarial attacks, although they are still more robust than CNNs with comparable complexities. For example, Swin-T/Swin-B suffer from a  and 14.90\%/5.04\% robust accuracy drop compared with DeiT-S/DeiT-B under PGD-20 attacks with a perturbation strength of 0.001, respectively; (3) the degree of overparameterization has less influence in the robustness for the same family of ViT models compared with its great influence to CNNs as the most lightweight DeiT-Ti can already achieve a comparable robust accuracy (-0.58\%) as ResNet-152 while requiring 9.17x/46x less floating-point operations (FLOPs)/parameters.
\textbf{Observations.} From the evaluation results summarized in Tab.~\ref{tab:sanity_check}, we make the following observations: (1) ViTs are consistently more robust than CNNs with comparable model complexities under all attack methods, which is consistent with the previous observations~\citep{bhojanapalli2021understanding, aldahdooh2021reveal, shao2021adversarial}. In particular, DeiT-S/DeiT-B achieves a 18.70\%/10.11\% higher robust accuracy over ResNet-50/ResNet-152 under PGD-20 attacks with a perturbation strength of 0.001; (2) compared with vanilla ViTs, ViT variants equipped with local self-attention or convolutional modules, which improves the model capability to capture local features and thus boosts the clean accuracy, are more vulnerable to adversarial attacks, although they are still more robust than CNNs with comparable complexities. For example, Swin-T/Swin-B suffers from a 14.90\%/5.04\% robust accuracy drop compared with DeiT-S/DeiT-B under PGD-20 attacks with a perturbation strength of 0.001; and (3) the degree of overparameterization has less influence in the robustness for the same family of ViT models compared with its great influence in CNNs' robustness, as the most lightweight DeiT-Ti can already achieve a comparable robust accuracy (-0.58\%) as ResNet-152, while  requiring 9.17$\times$/46$\times$ less floating-point operations (FLOPs)/parameters.


% Taking the three model variants in the DeiT family for example, their robust accuracy gap is within 12.19\% under PGD-20 attacks with a perturbation strength of 0.001, while the robustness gap between ResNet-18 and ResNet-152 is up to \NOTE{XX} under PGD-20 attacks. \NOTE{(What about Swin and LeViT?)}
    

% \textbf{Analysis.} Combining the three insights from the aforementioned observations, we can see the superiority of the global attention mechanism over convolutional and local self-attention blocks, in terms of both improved robust accuracy and less sensitivity to the model overparameterization. This indicates that the global attention mechanism itself can serve as a good robustification technique against existing adversarial attacks, even in lightweight ViTs with small model complexities. For example, as shown in Fig.~\ref{fig:patch_fool}, the gap between the attention maps generated by clean and adversarial inputs in deep layers keeps small. We wonder that "are the global attentions in ViTs truly robust, or their vulnerability has not been fully explored and exploited"? To answer this, we propose our customized attack in Sec.~\ref{sec:method}.
\textbf{Analysis.} Combining the three insights drawn from the aforementioned observations, we can observe the superiority of the global attention mechanism over convolutional and local self-attention blocks, in terms of both improved robust accuracy and reduced sensitivity to the degree of model overparameterization. This indicates that the global attention mechanism itself can serve as a good robustification technique against existing adversarial attacks, even in lightweight ViTs with small model complexities. For example, as shown in Fig.~\ref{fig:patch_fool}, the gap between the attention maps generated by clean and adversarial inputs in deeper layers remains small. We wonder that "Are the global attentions in ViTs truly robust, or their vulnerability has not been fully explored and exploited?". To answer this, we propose our customized attack in Sec.~\ref{sec:method}.

% To answer this question, we need to figure out the reason behind their robustness against existing adversarial attacks first. 


% \subsection{Why ViTs are more robust than CNNs?}
% \label{sec:understand}



